Social-Group-Agnostic Word Embedding Debiasing via the Stereotype Content Model

Existing word embedding debiasing methods require social-group-specific word pairs (e.g., "man"-"woman") for each social attribute (e.g., gender), which cannot be used to mitigate bias for other social groups, making these methods impractical or costly to incorporate understudied social groups in debiasing. We propose that the Stereotype Content Model (SCM), a theoretical framework developed in social psychology for understanding the content of stereotypes, which structures stereotype content along two psychological dimensions - "warmth" and "competence" - can help debiasing efforts to become social-group-agnostic by capturing the underlying connection between bias and stereotypes. Using only pairs of terms for warmth (e.g., "genuine"-"fake") and competence (e.g.,"smart"-"stupid"), we perform debiasing with established methods and find that, across gender, race, and age, SCM-based debiasing performs comparably to group-specific debiasing

==> sections/7-response.tex <==
% \section{Response}
% \begin{enumerate}
%     \item Replication with pretrained embedding
%     \item visualization to show how embeddings move
%     \item adding a few other social groups 
%     \item how to show def balance is preserved
% \end{enumerate}

% \textbf{Biggest thing to address: WHY DO WE NEED TO DEBIAS WORD EMBEDDINGS? ARE WE LOSING THE SENSE OF SOCIAL GROUPS IN THE PROCES?}

\noindent\textbf{Response to the Meta-Review:}
%We thank the meta-reviewer for their positive and constructive feedback on our paper. 
We appreciate the positive feedback, along with the assessment that our work is novel and that it would have broad applications. 
% The meta-reviewer raised concerns regarding: 1. having ``socially agnostic word embeddings'', 2. the fact that our method is specific to gender, and 3. that the fundamental motivations for the method were not laid out clear. 
First, we'd like to clarify that our claim was not that ``word embeddings should be socially agnostic''; rather, we claim that \textit{debiasing efforts} should proceed in a socially agnostic way. In Tables 1 and 2 in the paper, we demonstrate that debiasing along the two dimensions proposed by the Stereotype Content Model is a theory-driven method that is generalizable for multiple groups, compared to debiasing along individual social group dimensions. Next, we'd like to stress that our proposed method is not specific to gender; in our experiments it is evident that our method generalizes to other categories such as race, age, and physical appearance. 
%Then, we acknowledge that the motivation behind our methodology could have been described more thoroughly; however, 
We believe that the core components of our methodological motivations are present in the current paper. Overall, we make the case that (a) social-group biases in word embeddings are rooted in social stereotyping, and (b) debiasing embeddings along the dimensions of warmth and competence provides a more generalizable approach that is grounded in social scientific theory. 

%We acknowledge that our work on word embeddings needs to be extended to state-of-the-art language models to maximize the benefits of bias mitigation efforts, however, this work could be a an the first theory-driven step in that direction.

%Lastly, we also clarify our definition of bias. Conceptually, social group biases in word embeddings are instances of representational harms \cite{suresh2021framework, crawford2017trouble}. %Representational harms happen when groups are stereotyped or stigmatized. 
%Section 3.3 discusses the measurements of bias we have used in this work. 



\noindent\textbf{Response to Reviewer 1:}
%In response to concerns about our motivation (i.e., focusing on concrete harm), Given the ubiquity of word embeddings in sensitive industry applications, any means of improving such embeddings' fairness is worth pursuing. Indeed, in our paper we strongly motivate the idea that 
%we would like to clarify that word embedding models are still widely used at production settings for various purposes ranging from simple text completion to document retrieval. Most of these applications operate based on some notion of distance between words. 
%stereotypically biased word embedding models are more likely to yield stereotypical responses, hence perpetuating undesirable stereotypes for minorities in many cases. Debiasing efforts, such as ours, aim to prevent perpetuating such biases at scale. 
In response to the concern that our work might suffer from the the same issues reported by \citeauthor{gonen2019lipstick} (\citeyear{gonen2019lipstick}), we point out that, in contrast to previous work that mitigates and measures bias along the same subspace (e.g., mitigating bias on gender and measuring improvements on gender), our method is evaluated along multiple subspaces (i.e., age, gender, and race) which are not directly related to the proposed theory-driven bias mitigation subpspace (i.e., warmth and competence). %Further, given that in our work a. there are multiple evaluation dimensions involved rather than one, and b. that these dimensions are not aligned with neither warmth nor competence,
This significant difference in our approach is evidence for why the proposed operations are not only at a superficial level. We will add the relevant citations mentioned by the reviewer to the final submission and have addressed some of the reviewer's concern in the limitations section. 

\input{tables/rebuttal-v2}

\noindent\textbf{Response to Reviewer 2}:
%We appreciate the reviewer's positive comments and helpful critiques. 
First, in response to the question ``[S]hould people really be somewhere in the middle between pleasant and unpleasant,'' we respectfully hope that the reviewer agrees that representing social groups as equally ``pleasant,'' which our method attempts to achieve, is a step forward towards building more egalitarian representations. If the reviewer is concerned about removing the social identity of the groups, we point out that the work of \citet{dev2019attenuating} on partial projection, on which our main experiments are based, preserves some definitional bias by
%aims to preserve some amount of definitional bias, which is orthogonal to the bias subspace.
%This work 
regulating the amount of debiasing based on the norm of the representation along and orthogonal to the bias dimension. Regarding the question as to whether ``word embedding benchmarks used in this study actually evaluate for the preservation of definitional bias [...]'' we point to the content of the \href{http://download.tensorflow.org/data/questions-words.txt}{Google analogy evaluation}, half of which contains categories such as family, currency, and capitals of countries. These represent part of groups' definitional bias. 
% As far as our work is concerned, we, similarly aim to remove unintended bias while preserving definitional bias.
 To the reviewer's question regarding the statistical significance of results in Table 1, we reference section 4.1, lines 288 to 291.
% , in which we state that ``All methods were repeatedly applied using 30 different word pair samples, and we report each measure’s average and compare values using 95\% confidence intervals.'' 
%\textbf{Is this removing the def bias}
%We point the reviewer to evidence that strongly suggests that our method is not completely removing the social identity of the social groups
%{\color{red}Visualization and Valence}

%To an extent yes, The empirical evidence for our claim can be found in the utility evaluations of section 4.2 (table 2). For example google analogy (link here ) includes categories such as family, currency and capitals of the world that are related to the definitonal bias of the categories In fact almost half of this dataset is comprised of such analogies. Specifically compared to removing categories one by one our method does better. 


\noindent\textbf{Response to Reviewer 3: }
% We thank Reviewer 3 for their comments. We believe these comments can be 
% \textbf{Typos and same confusion}
%We thank Reviewer 3 for their positive feedback. 
The typos and confusions in wording will be addressed in our final submission.
% and we appreciate the reviewer's attention to the details.
%We will fix the typo on line 452. Regarding the confu and change the caption of table \textbf{zzz} to clarify the same dimension confusion
%we established baselines by applying HD, Sub, LP, and PP using the respective word pair list (e.g., for gender bias we used gender word pairs), denoted with the subscript ``same.''
% \textbf{Beyond Race/Gender/Age}
In response to the requests for (1) replicating our results with pretrained embeddings, and (2) including additional social groups, %and (3) to address the concern about generalizability of our method to pretrained embeddings, 
we present our results for \href{https://code.google.com/archive/p/word2vec/}{Word2Vec trained on Google News}
% two prominent social groups in the US namely 
including additional groups of Asians, Hispanics, and fat vs. thin (Table \ref{tab:rebuttal}). The results show that our proposed framework succeeds in handling these additional dimensions and generalizes to other embeddings.  




% additional analysis that plan to incorporate this in our final submission. We added comparison of bias for additional social groups such as . In addition we also included physical appearance (i.e. fat-thin) and tested our proposed approach. The results may be found in ....

% Tessa's work is here https://osf.io/th89x/ it includes list of social group term, I'll add a few social groups (let's hope it works!)




% We additionally will add a supplemental analysis, in which we repeated the experiments with the Word2Vec model, pretrained on Google News. The result was consistent with our previously reported results. %We replicated our analysis using the Google news pretrained embedding model \textbf{cite} the results are \textbf{consistent} with our previous analysis. Table ... shows the same metrics. 











% \textbf{Gonen and Goldberg (NBM) - I don't know how to deal with this} put in limitations







==> sections/style_guide.tex <==
\begin{abstract}
This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences. 
The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/docs/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

% Entries for the entire Anthology, followed by custom entries
\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\section{Example Appendix}
\label{sec:appendix}

This is an appendix.

